Heterogeneous earning responses to inheritance: new event-study evidence from Norway

It has long been assumed that inheritances, particularly large ones, have a negative effect on the labor supply of inheritors. Using Norwegian registry data, I examine the inheritance-induced decline in inheritors' wages and occupational income. In contrast to prior research, my estimates allow the dynamic effect of inheritances on labor supply to vary among inheritor cohorts. The estimation approach adopted and the 25-year long panel data make it possible to trace the dynamics of the effect for at least 20 years, which is twice as long as the study period in previous studies. Since all observations in the sample are inheritors, I avoid the selection problem arising in studies employing non-inheritors as controls. I find that large parental inheritances (more than one million Norwegian kroner) reduce annual wage and occupational income by, at most, 4.3%, which is about half the decrease previously identified. The magnitude of the effect increases with the size of the inheritance. Large inheritances also increase the probability of being self-employed by more than 1%, although entrepreneurship may be dampened by inheritances that are excessively large. The inheritance effect lasts for up to 10 years and is heterogeneous across sexes and age groups. Male heirs are more likely to reduce their labor supply after receiving the transfer. Young heirs are more likely to be self-employed, and their annual occupational income is, therefore, less affected by inheritances in the long run; for the very young inheriting large amounts of wealth from their grandparents, the probability of their attaining a post-secondary education declines by 2%.

==> tables/age_constraint.tex <==
\begin{table}[htbp]\centering

\caption{Different age constraints in my study and in the literature}
\label{tab:age_constraint}
\vspace{-5pt}
 
\begin{threeparttable}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|cc|c|c|c|c|c|c|}
\cline{2-19}   
Birth    &19&19&19&19&19&19&19&19&19&19& \multirow{2}{*}{$\cdots$}& \multirow{2}{*}{$\cdots$}    &19&19&19&19&19&19    \\  [-0.3em]
year     &44&45&46&47&48&49&50&51&52&53&                        &                            &73&74&75&76&77&78    \\  \cline{2-19} 
baseline &  &  &  &  &  &  &  & \multicolumn{8}{c}{\cellcolor{black!70}}                            &  &  &    \\  \cline{2-19} 
Boe     &        \multicolumn{16}{c}{\cellcolor{blue!70}}                                            &  &      \\  \cline{2-19} 
relaxed  &  &  &  &  &  \multicolumn{14}{c}{\cellcolor{red!70}}                                  \\  \cline{2-19} 
\end{tabular}
\begin{tablenotes}
      \small  
      \item \quad \quad \quad \quad \quad  Note: ``baseline'' is the default age constraint in my study; ``Boe'' is the sample age constraint in \cite{Boe2019};
      \item \quad \quad \quad \quad \quad  ``relaxed'' is an eased age constraint as a robustness check.
    \end{tablenotes}
\end{threeparttable}
\end{table}




==> tables/des_collapse.tex <==
\begin{table}
\caption{Sample mean between 1993 and 2017 by inheritance size}
\vspace{-7pt}
\scalebox{0.9}{
\begin{tabular}{l*{5}{c}}
\toprule
Interval &all&I1&I2&I3&I4 \\
\midrule
labor income&        379&      343&      363&      385&      426\\
occupational income&  406&      374&      391&      414&      466 \\
entrepreneurship&   0.13 &  0.14    &  0.12    &    0.12 &  0.13    \\
capital income&       29&       18&       20&       27&       60\\
transfer    &         40&       42&       41&       39&       35\\
gross wealth&        836&      634&      676&      811&    1,384\\
gross debt  &        602&      549&      564&      608&      721\\
\midrule
Obs.  & 140,279& 42,592&34,532&34,177 &28,978 \\
\bottomrule
\multicolumn{6}{l}{\footnotesize Note: Income and wealth are deflated with CPI to $1,000$ NOK in 2015}\\
\end{tabular}}
\end{table}


==> tables/des_event.tex <==
\scalebox{1}{
\begin{table}[htbp]
\begin{threeparttable}
% \caption{Sample mean in event year $E_i$ by inheritance size \vspace{-7pt}}
\begin{tabular}{l*{5}{c}}
\toprule
Interval &all&I1&I2&I3&I4 \\
\midrule
inheritance year&         2007&    2005&    2006&    2008&    2009\\
inheritance amount&      568&      102&      272&      548&    1,691\\
labor income&            398&      348&      382&      416&      470\\
occupational income&     430&      379&      410&      447&      513\\
$Pr($self-employment$)$&        0.14&         0.15&         0.13&       0.13&        0.14\\
capital income&           36&       17&       22&       36&       83\\
gross wealth&          1,146&      638&      817&    1,129&    2,369\\
-financial wealth&      436&      211&      293&      436&      965\\
-housing wealth&        252&      177&      215&      261&      402\\
-gross debt &           655&      556&      608&      687&      829\\
-debt rate  &          0.57&      0.87&     0.74&        0.61&  0.35 \\
age         &             47&       45&       46&       48&       49\\
male        &              0.47&        0.47&        0.47&        0.47&        0.49\\
education   &              4.24&        4.00&        4.12&        4.28&        4.69\\
married     &              0.78&        0.75&        0.77&        0.80&        0.80\\
number of kids&            0.99&        1.11&        0.99&        0.90&        0.91\\
paternal death&            0.79&        0.74&        0.77&        0.82&        0.86\\
maternal death&            0.62&        0.53&        0.58&        0.67&        0.75\\

\midrule
no. of individuals  & 120,952& 36,972&29,783&34,177 &23,924 \\
% \midrule
% \textcolor{gray}{Obs. (any time)} & \textcolor{gray}{271,407}& \textcolor{gray}{108,516}&\textcolor{gray}{70,504}&\textcolor{gray}{55,416} &\textcolor{gray}{36,971} \\
\bottomrule
\end{tabular}
\begin{tablenotes}
      \small
      \item Note: Income and wealth are deflated with CPI to $1,000$ NOK at 2015 price.
    \end{tablenotes}
\end{threeparttable}
\end{table}}
